A new Truncated Fourier Transform algorithm

Truncated Fourier Transforms (TFTs), first introduced by Van der Hoeven, refer to a family of algorithms that attempt to smooth "jumps" in complexity exhibited by FFT algorithms. We present an in-place TFT whose time complexity, measured in terms of ring operations, is comparable to existing not-in-place TFT methods. We also describe a transformation that maps between two families of TFT algorithms that use different sets of evaluation points.

==> cooley_tukey_short2.tex <==
\subsection{The Fast Fourier Transform}

We can compute the discrete Fourier transform of $f(z)$, $f$ reduced modulo $(z^n-1)$, by way of a {\em Fast Fourier Transform} (FFT).  The FFT is believed to have been first discovered by Gauss, but did not become well-known until it was famously rediscovered by Cooley and Tukey \cite{CT}.  For a detailed history of the FFT we refer the reader to \cite{history}.

There are many variants of the FFT.  We describe the {\em radix-2} Cooley-Tukey FFT in terms of modular reductions.   Let $n$ be a power of two.  We break $f$ into images modulo polynomials of decreasing degree until we have the images $f \bmod (z-\omega^i) = f(\omega^i)$, $0 \leq i < n$.  At the start of the first iteration we have $f$ reduced modulo $z^n-1$.  After $i$ iterations, we will have the $2^i$ images
\begin{equation}
f \bmod z^{u}-\omega^{ju}, \hspace{0.4cm}\text{ for } 0 \leq j < n/u.
\end{equation}
If $i=\log_2 n$ this gives us the DFT of $f$.  Consider then the image $f' = f(z) \bmod z^{2u} - \omega^{2ju} = \sum_{i=0}^{2u-1}b_i$, for some $j$, $0 \leq j < \tfrac{n}{2u}$.  We break this image into two images $f_0$ and $f_1$, where
\begin{align}
f_0 &= f' \bmod (z^{u} - \omega^{ju}), \text{and} \\
f_1 &= f' \bmod (z^{u} + \omega^{ju}) = f' \bmod (z^u - \omega^{ju + n/2}),
\end{align}
If we write $f' = \sum_{k=0}^{u-1}b_kz^k$, then we can write $f_0$ and $f_1$ in terms of the coefficients $b_k$:
\begin{equation}
f_0 = \sum_{k=0}^{u-1}(b_k + \omega^{v}b_{k+u} )z^k, \hspace{0.4cm} f_1 = \sum_{k=0}^{u-1}(b_k - \omega^{v}b_{k+u})z^k.
\end{equation}
thus, given an array containing the coefficients $b_k$ of $f'$, we can write $f_0$ and $f_1$ in place of $f'$ by way of operations
\begin{equation}\label{eqn:rad2fft}
(b_k, b_{k+u}) \leftarrow (b_k + \omega^{ju}b_{k+u}, b_k - \omega^{ju}b_{k+u}), \hspace{0.4cm} 0 \leq i \leq u
\end{equation}
The pair of assignments \eqref{eqn:rad2fft} are known as a {\em butterfly operation}.  Note $f_0$ and $f_1$ are in the same form as $f'$, and if $u>1$ we can break those images into smaller images in the same fashion.  Starting this method with $f \bmod (z^n-1)$, will give us $f \bmod (z-\omega^j) = f(\omega^j)$, for $0 \leq j < n$.

If the butterfly operations are performed in place, the resulting evaluations $f(\omega^j)$ will be written in {\em bit-reversed} order.  More precisely, if we let $\rev_c(j)$ denote the integer resulting from reversing the first $c$ bits of $j$, we have that $f(\omega^j)$ will be written in place of $a_{k}$, where $k=\rev_{\log(n)}(j)$ and $\log$ is taken to be base-2 throughout.  As an example,
\begin{equation}
\rev_5(11) = \rev_5({\tt 01011}_2) = {\tt 11010}_2 = 16+8+2=26.
\end{equation}

\begin{procedure}
	\caption{FFT(\textbf{a}, $n$, $\omega$), an in-place implementation of the radix-2 Cooley-Tukey FFT}\label{proc:FFT}
	\KwIn{
		\begin{itemize}[noitemsep,nolistsep]
			\item  $\textbf{a} = (\textbf{a}(0), \dots, \textbf{a}(n-1))$, an array containing a vector $a \in\mathcal{R}^n$.
			\item  $\omega$, a root of $z^n-1$, for $n$ a power of two.
		\end{itemize}
	}
	\KwResult{ $\DFT_\omega^n(a)$ is written to the array ${\bf a}$ in bit-reversed order.  }\vspace{0.3cm}
	
	\For{$i \longleftarrow 1$ \KwTo $\log_2(n)$}{
		%$m \longleftarrow n/2^i$\\
		$u \longleftarrow n/2^i$\\
		
		\For{$j \longleftarrow 0$ \KwTo $\tfrac{n}{2u}-1$}{
			$t \longleftarrow \rev_i(j)u$\\
			%
			\For{$k \longleftarrow 0$ \KwTo $u-1$ }{
				\tcp{Butterfly operations \eqref{eqn:rad2fft}} 
				$\left[\begin{matrix} {\bf a}(t+k) \\ {\bf a}(t+k+u)\end{matrix}\right] \longleftarrow \left[\begin{matrix} 1 & \omega^{ju} \\ 1 & -\omega^{ju}\end{matrix}\right]\left[\begin{matrix} {\bf a}(t+k) \\ {\bf a}(t+k+u)\end{matrix}\right]$ \\
				\label{line:butterfly}
			}
			%$\gamma \longleftarrow \gamma\zeta$\label{line:powers}\\
		}
	}
\end{procedure}

\begin{procedure}
	\caption{IFFT(\textbf{a}, $n$, $\omega$), an in place implementation of the inverse-FFT }\label{proc:IFFT}
	\KwIn{ $\textbf{a} = (\textbf{a}(0), \dots, \textbf{a}(n-1))$, an array containing $\DFT_{\omega}^n(a)$, for a vector $a \in \mathcal{R}^n$, for $n$ a power of two, in bit-reversed order.
	}
	\KwResult{ The vector $a$ is written to array ${\bf a}$ in place of its DFT. }\vspace{0.3cm}
	
	\For{$i \longleftarrow 1$ \KwTo $\log_2(n)$}{
		$u \longleftarrow n/2^i$\\
		%$m \longleftarrow 2^{i-1}$\\
		
		%\For{$j \longleftarrow 0$ \KwTo $\tfrac{n}{2m}-1$}{
		\For{$j \longleftarrow 0$ \KwTo $\tfrac{n}{2u}-1$}{
			$t \longleftarrow \rev_{i}(j)\tfrac{n}{2u}$\\
			\For{$k \longleftarrow 0$ \KwTo $u-1$}{
				\tcp{Butterfly operations \eqref{eqn:rad2fft}}				
				$\left[\begin{matrix} {\bf a}(t+\tfrac{kn}{u} ) \\ {\bf a}( t+\tfrac{kn}{u}+ \tfrac{n}{2u}) \end{matrix}\right] \longleftarrow
				\left[\begin{matrix} 1 & \omega^{-ju} \\ 1 & -\omega^{-ju}\end{matrix}\right]$
				$\left[\begin{matrix} {\bf a}(t+\tfrac{kn}{u} ) \\ {\bf a}( t+\tfrac{kn}{u}+ \tfrac{n}{2u}) \end{matrix}\right]$
		
			}
		}
	}\vspace{0.3cm}
	
	\lFor{$i \longleftarrow 0$ \KwTo $n-1$}{ $\textbf{a}(i) \longleftarrow \tfrac{1}{n}{\bf a}(i)$ }
	
\end{procedure}

Procedures {\tt\ref{proc:FFT}} and {\tt\ref{proc:IFFT}} describe implementations of this in-place FFT and its inverse.  {\tt\ref{proc:IFFT}} computes the inverse as $\tfrac{1}{n}\DFT_\omega^n$, and requires that the input is in bit-reversed order.

Normally one would pre-compute powers of $\omega$ and store them in an array in bit-reversed order.  To avoid this space overhead we perform the butterfly operations in an order such that we can compute the required powers of $\omega^m$ sequentially.  For better memory performance, one can produce the powers of $\omega$ in an order that allows us to traverse the array in sequential order, at the cost of an additional $\mathcal{O}(n)$ ring multiplications.

Our only ring operations required are those in butterfly operations (line \ref{line:butterfly}) and the computation of the powers of $\omega^{ju}$.  $\omega^u$ can be computed by a square-and-multiply approach using $\mathcal{O}(\log u)$ multiplications.  Enumerating these operations gives us the following cost:

\begin{lem}
Let $n$ be a power of two and let ${\bf a}$ be an array containing the coefficients of a polynomial $f(z)$ reduced modulo $(z^n-1)$.  Computing $\DFT_{\omega}^n(a)$ by way of procedure {\tt\ref{proc:FFT}}, requires $n\log n + \mathcal{O}(1)$ additions and $\tfrac{1}{2}n\log n + \mathcal{O}(n)$ multiplications in $\mathcal{R}$.  Procedure ${\tt\ref{proc:IFFT}}$ has similar complexity.
\end{lem}

The approach described for $n$ a power of two generalizes for $n$ a prime power or a product of small primes, though in practise $n$ is almost always chosen to be a power-of-2.

Using the radix-2 FFT, if $d = \deg(fg)$, we choose $n$ to be the least power of $2$ exceeding $d$.  This entails appending zeros to the input arrays $a$ and $b$.  By this method, computing a product of degree $2^k$ requires the same time and space cost as computing a product of degree $2^k+m$, for $0 \leq m < 2^k$.  It would be preferable to have a radix-2 FFT algorithm whose time cost grows smoothly relative to $n$, and which requires $n+\mathcal{O}(1)$ space for arbitrary integers $n>0$, and not just for $n$ a power of two.  Crandall's {\em devil's convolution} algorithm \cite{scicomp} somewhat flattens these jumps in complexity, though not entirely.  It works by reducing a discrete convolution of arbitrary length into more easily computable convolutions.  More recently, truncated Fourier transform (TFT) algorithms, described hereafter, have addressed this issue.


==> dft_short.tex <==

\subsection{The discrete Fourier transform and its inverse}

The {\em discrete Fourier transform} (DFT) of a polynomial $f(z)$ is its vector of evaluations at the distinct powers of a root of unity.  Specifically, if $f(z) = \sum_{i=0}^{n-1}a_iz^i$ is a polynomial over a ring $\mathcal{R}$ containing an $n\th$ primitive root of unity $\omega$, then we define the discrete Fourier transform of $f(z)$ as
\begin{equation}
\DFT^n_\omega( f ) = \left( f(\omega^j) \right)_{0 \leq j < n }.
\end{equation} 
We treat the polynomial $f$ and its vector of coefficients $a  = ( a_0, a_1, \dots, a_{n-1} )$ as equivalent and use the notation $\DFT_\omega^n( a )$ and $\DFT_\omega^n( f )$ interchangeably.  If we take addition and multiplication to be pointwise in $\mathcal{R}^n$, then the map $\DFT_\omega^n:\mathcal{R}[z]/(z^n-1)\rightarrow \mathcal{R}^n$ forms a ring homomorphism.  If $\omega$ is a {\em principal} root of unity, that is, for $j$ not divisible by $n$, $\sum_{i=0}^{n-1} \omega^{ij} = 0$,
then, $\DFT_\omega^n$ has an inverse map $\IDFT^n_{\omega} : \mathcal{R}^n \rightarrow \mathcal{R}[z]/(z^n-1)$, defined by
\begin{equation}
\IDFT^n_{\omega}( \hat{a} ) = \tfrac{1}{n}\DFT_{\omega^{-1}}( \hat{a} ),
\end{equation}
where $\hat{a} \in \mathcal{R}^n$ and we again we treat a polynomial as equivalent to its vector of coefficients.  This suggests a multiplication algorithm for $f,g \in \mathcal{R}[z]$.
\begin{thm}[The Convolution Theorem]
Suppose $\mathcal{R}$ is a ring containing an $n\th$ principal root of unity $\omega$ and let $f,g \in \mathcal{R}[z]$.  Then
\begin{equation}
fg \bmod (z^n-1) = \IDFT_\omega^n\left( \DFT_\omega(f)\cdot \DFT_\omega(g) \right),
\end{equation}
where ``$\cdot$'' is the vector dot-product, and, given two polynomial $g(z), h(z) \in \mathcal{R}[z]$, $g(z) \bmod h(z)$ denotes the unique polynomial $r(z)$ such that $h(z)$ divides $g(z)-r(z)$ and $\deg(r)<\deg(h)$ throughout.
\end{thm}
Thus to multiply $f$ and $g$, we can choose $n>\deg(fg)$ and an $n\th$ principal root of unity $\omega \in \mathcal{R}$, compute the length-$n$ DFTs of $f$ and $g$, take their pointwise product, and take the inverse DFT of the result.  If $\mathcal{R}$ does not contain such a root of unity $\omega$, we can choose $n>\deg(fg)$ such that $n$ and the characteristic of $\mathcal{R}$ are relatively prime and instead use the ring $\mathcal{R}[w]/(w^n-1)$ containing $n\th$ principal root of unity $w$.
